Fast greedy algorithms for dictionary selection with generalized sparsity constraints

In dictionary selection, several atoms are selected from finite candidates that successfully approximate given data points in the sparse representation. We propose a novel efficient greedy algorithm for dictionary selection. Not only does our algorithm work much faster than the known methods, but it can also handle more complex sparsity constraints, such as average sparsity. Using numerical experiments, we show that our algorithm outperforms the known methods for dictionary selection, achieving competitive performances with dictionary learning algorithms in a smaller running time.

==> gap.tex <==
%!TEX root=./main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Gap between Dictionary Selection and Dictionary Learning}\label{sec:dictlearn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we analyze a theoretical gap between dictionary learning and dictionary selection.
Recall that in dictionary learning, all the unit vectors are possible atoms, and therefore we cannot apply dictionary selection algorithms directly. 
In the following, we fix a dictionary with normalized columns $\bD^* \in \R^{d\times k}$.
Let $f_t \colon \R^{d \times k} \to \R$ be $f_t(\bD) = \max_{\bw\colon \norm{\bw}_0 \leq s} u(\by_t, \bD\bw)$.
We define the distance between two dictionaries $\bD$ and $\bD'$ by $d(\bD, \bD') = \max_i \min_j \norm{\bd_i \pm \bd'_j}_2^2$, where $\bd_i$ and $\bd'_i$ are the $i$th column of $\bD$ and $\bD'$, respectively.
The following lemma relates the regret in online dictionary selection to that in online dictionary learning. 

We need some notations to state the lemma.
Let $\bA \in \R^{d \times n}$ be a fixed matrix with normalized columns, and denote by $\bar{\bD} \in \R^{d \times k}$ a column submatrix of $\bA$ minimizing $d(\bar{\bD}, \bD^*)$.
For $t \in [T]$, let $\bw^*_t \in \argmax_{\bw: \norm{\bw}_0 \leq s} u(\by_t, \bD^*\bw)$ and define $\bar{\bw}_t$ similarly for $\bar{\bD}$.
Define $\Theta_t \subseteq \R^d$ as the convex hull of four points $\bD^*\bw^*_t$, $\bD^*\bar\bw_t$, $\bar\bD\bw^*_t$, and $\bar\bD\bar\bw_t$ for $t \in [T]$.

\begin{theorem}\label{thm:discretization}
	Assume that $u(\by_t, \bx)$ is Lipschitz continuous in $\bx$:
    there exists a constant $L > 0$ such that
    	$\abs{u(\by_t, \bx) - u(\by_t, \bx')} \leq L \norm{\bx - \bx'}_2$ for arbitrary $\bx, \bx' \in \Theta_t$ and $t \in [T]$.
    Let $\bD_t$ be the outputs of an online dictionary selection algorithm with the columns in $\bA$ being the ground set. 
    Then 
    \begin{align*}
   		\alpha &\sum_{t=1}^T f_t(\bD^*) - \sum_{t=1}^T f_t(\bD_t) \\
        &\leq 
        r_\alpha(T) + \alpha LTM\left[ \sqrt{s\epsilon} + 2\sigmamax(\bar\bD, 2s) \right],
    \end{align*}
    where $d(\bD^*, \bar\bD) \leq \epsilon$, $r_\alpha(T)$ is the $\alpha$-regret of the dictionary selection algorithm, and $M \geq \max_t \max \{ \norm{\bw^*_t}_2, \norm{\bar\bw_t}_2 \}$.
\end{theorem}

\begin{proof}
Let us fix $t \in [T]$ arbitrary.
For $\by_t$, let $\bw_t^*, \bar{\bw}_t \in \argmin_{\bw\colon \norm{\bw}\leq s} u(\by_t, \bD\bw)$ for $\bD = \bD^*$ and $\bar\bD$, respectively.
Then,
\begin{align*}
	&u(\by_t, \bD^*\bw_t^*) \\
    &= u(\by_t, \bar{\bD}\bar{\bw}_t - (\bar{\bD} - \bD^*)\bw^*_t + \bar{\bD}(\bw^*_t - \bar{\bw}_t)) \\ 
    &\leq u(\by_t, \bar{\bD}\bar{\bw}_t) 
    + L \norm{(\bar{\bD} - \bD^*)\bw^*_t + \bar{\bD}(\bw^*_t - \bar{\bw}_t)}_2  \tag{by the Lipschitz continuity of $u$}\\ 
    &\leq u(\by_t, \bar{\bD}\bar{\bw}_t) 
    + L \norm{(\bar{\bD} - \bD^*)\bw^*_t}_2 + L \norm{\bar{\bD}(\bw^*_t - \bar{\bw}_t)}_2.  \tag{by the triangle inequality} 
\end{align*}
Since $\bw^*_t$ is $s$-sparse, $\norm{(\bar{\bD} - \bD^*)\bw^*_t}_2 \leq \sqrt{s\epsilon}M$.
On the other hand, $\norm{\bar{\bD}(\bw^*_t - \bar{\bw}_t)}_2 \leq \sigmamax(\bar{\bD}, 2s)\norm{\bw^*_t - \bar\bw_t}_2 \leq \sigmamax(\bar{\bD}, 2s) \cdot 2M$.
Thus, 
\begin{align*}
	u(\by_t, \bD^*\bw^*) \leq 
    u(\by_t, \bar{\bD}\bar{\bw}_t) + LM(\sqrt{s\epsilon} + 2\sigmamax(\bar{\bD},2s))
\end{align*}
for $t \in [T]$.
Therefore, 
\begin{align*}
	&\alpha \sum_{t=1}^T u(\by_t, \bD^*\bw^*_t) \\
	&\leq \alpha \sum_{t=1}^T u(\by_t, \bar{\bD}\bar{\bw}_t) + \alpha LMT(\sqrt{s\epsilon} + 2\sigmamax(\bar{\bD},2s)) \\
	&\leq \alpha \sum_{t=1}^T u(\by_t, \bD_t\bw_t) + \alpha LMT(\sqrt{s\epsilon} + 2\sigmamax(\bar{\bD},2s)) + r_{\alpha}(T), 
\end{align*}
where $\bw_t \in \argmin_{\bw\colon \norm{\bw}_0 \leq s} u(\by_t, \bD_t \bw)$ for $t \in [T]$.
By the definition of $f_t$, we obtain the desired bound.
\end{proof}


\begin{corollary}
Let $u$ be the squared $\ell^2$-utility function.
Assume that there exists $D > 0$ such that
$\norm{\by_t}_2 \leq D$ for $t \in [T]$. 
Then $L \leq 2\max\{\sigmamax(\bD^*, s), \sigmamax(\bar\bD, s)\}M$ and $M \leq D/\min\{\sigmamin(\bD^*,s), \sigmamin(\bar\bD, s)\}$.
\end{corollary}

In the rest of this section, we focus on the squared $\ell^2$-utility function. 
A natural approach for reducing dictionary learning to dictionary selection is to take a discretization of the unit sphere. 
A finite subset $U$ of the unit sphere is called an \emph{$\epsilon$-net} for $\epsilon > 0$, if for any unit vector $\bx$, there exists $\by \in U$ such that $\norm{\bx - \by}^2_2 \leq \epsilon$.

\begin{definition}
	Let $\bA \in \R^{d \times n}$ be a matrix with normalized columns.
    The \emph{coherence} of $\bA$ is defined as 
    \begin{align}
    \mu = \max_{i \neq j} \abs{\inprod{\ba_i, \ba_j} },
    \end{align}
    where $\ba_i$ is the $i$th column of $A$.
    For a positive integer $s$, the \emph{restricted isometry constant (RIP constant)} $\delta_s$ with respect to $s$ is the smallest number such that 
    \begin{align}
    (1-\delta_s)\norm{\bx}_2^2 \leq \norm{\bA\bx}_2^2 \leq (1+\delta_s)\norm{\bx}_2^2,
    \end{align}
    for all $\bx \in \R^m$ with $\norm{\bx}_0 \leq s$.
%    The \emph{restricted condition number} $\kappa_s$ with respect to $s$  is defined as 
%    \begin{align}
%    	\kappa_s \coloneqq \max_{X \subseteq[n]\colon \abs{X} \leq s} \frac{\sigmamax(\bA_X)}{\sigmamin(\bA_X)}.
%    \end{align}
\end{definition}

It is well-known that $\mu \leq \delta_s \leq s \mu$ and $\frac{\sigmamax(\bA, s)}{\sigmamin(\bA,s)} \leq \sqrt{\frac{1+\delta_s}{1-\delta_s}}$ (see \citet{Foucart2013} for example).
From this perspective, an $\epsilon$-net has the coherence $1-\epsilon/2$, and therefore $\frac{\sigmamax(\bA, s)}{\sigmamin(\bA,s)}$ can be arbitrary large unless $s$ is a constant.
This makes the approximate-regret guarantees in \Cref{thm:modular-approx,thm:online-replacement-greedy} trivial.

The following shows that for a certain range of $d$, $k$, $n$ and $s$,  we can take a discretization with high probability that preserves the utility approximately with controlled dependence on the restricted condition number.

\begin{proposition}\label{thm:gap}
Let $\epsilon, \delta > 0$ and $p \in (0,1)$ be fixed constants and $\bD \in \R^{d \times k}$ be a fixed dictionary.
Let $\tilde\bA \in \R^{d \times n}$ be a random matrix whose entries are the standard Gaussians and $\bA$ be the matrix obtained by normalizing columns of $\tilde\bA$.
If $2n(\epsilon - \epsilon^2/4)^{d/2} - \log{k} \geq \log(2/p)$ and $d \geq \frac{C}{\delta^2}(s\log(n/s) + \log(4/p))$ for some constant $C \approx 80.98$,  then $\bA$ satisfies the following two conditions, with probability at least $1-p$:
(i) $\delta_s \leq \delta$, and 
(ii) there exists a submatrix $\bD' \in\R^{d\times k}$ of $\bA$ such that $d(\bD, \bD') \leq \epsilon$.
\end{proposition}

\begin{proof}
Let $\ba_1, \dots, \ba_n \in \R^d$ be the columns of $\bA$.
First, observe that for any fixed $\bd\in S^{d-1}$, the probability of $\abs{\inprod{\ba_i, \bd}} \geq 1 - \epsilon/2$ is the twice of the fraction of spherical area of the set $\{ \bx \in S^{d-1} \colon \inprod{\ba_i, \bd} \geq 1-\epsilon/2 \}$, which is at least $2 (\epsilon-\epsilon^2/4)^{d/2}$.
Let $\bd_1, \dots, \bd_k \in \R^d$ be the columns of $\bD^*$.
Then 
\begin{align*}
	\Pr\left(\max_{i=1}^n \abs{\inprod{\ba_i, \bd_j}} < 1- \epsilon/2 \right) \leq (1 - 2 (\epsilon-\epsilon^2/4)^{d/2})^n \leq \exp(-2n(\epsilon-\epsilon^2/4)^{d/2}).
\end{align*}
By the union bound,
\begin{align*}
	\Pr\left(\bigvee_{j=1}^k [\max_{i=1}^n\abs{\inprod{\ba_i, \bd_j}} < 1- \epsilon/2] \right) \leq k \exp(-2n(\epsilon-\epsilon^2/4)^{d/2}) = \exp(\log k -2n(\epsilon-\epsilon^2/42)^{d/2}).
\end{align*}
Therefore, by the assumption of the theorem, the probability of the condition (i) is violated is at most $p/2$.

On the other hand, it is known (see~\citet{Foucart2013}, for example) that if $d \leq \frac{C}{\delta^2}\left( s\log(en/s) + \log(4/p) \right)$, then $\delta_s(\bA) \leq \delta$ with probability at least $1-p/2$.
Therefore, the conditions (i) and (ii) are both satisfied with probability at least $1-p$.

\end{proof}

%\begin{corollary} 
%Let $\bD^* \in \R^{d \times k}$ be an arbitrary dictionary.
%Assume that $u(\by,\bx):= \norm{\by}_2^2 - \norm{\by - \bx}_2^2$ and  $\bw_t \in \argmin_{\bw : \norm{\bw}_0 \leq s} u(\by_t , \bD^*\bw)$ satisfies $\norm{\bw}_\infty \leq M$ for $t \in [T]$.
%If the assumption in Theorem~\ref{thm:gap} is satisfied, then the output of Algorithm~\ref{alg:online-replacement} with atoms $\bA$ satisfies that 
%\end{corollary}

